LawBreaker: An Approach for Specifying Traffic Laws and Fuzzing Autonomous Vehicles

Autonomous driving systems (ADSs) must be tested thoroughly before they can be deployed in autonomous vehicles. High-fidelity simulators allow them to be tested against diverse scenarios, including those that are difficult to recreate in real-world testing grounds. While previous approaches have shown that test cases can be generated automatically, they tend to focus on weak oracles (e.g. reaching the destination without collisions) without assessing whether the journey itself was undertaken safely and satisfied the law. In this work, we propose LawBreaker, an automated framework for testing ADSs against real-world traffic laws, which is designed to be compatible with different scenario description languages. LawBreaker provides a rich driver-oriented specification language for describing traffic laws, and a fuzzing engine that searches for different ways of violating them by maximising specification coverage. To evaluate our approach, we implemented it for Apollo+LGSVL and specified the traffic laws of China. LawBreaker was able to find 14 violations of these laws, including 173 test cases that caused accidents.

==> Fuzzing_Backup.tex <==
\section{Law Breaking Fuzzing}
\todo{SJ: Rewrite this part to present only one fuzzing algorithm, i.e., law-breaking fuzzing, based on generating a variety way of breaking the given law.}

In this section, we present two algorithms that we employ to evaluate whether the relevant and ready to be tested traffic rules are violated by existing ego vehicle controlling algorithms. The two feedback-guided fuzzing algorithms we proposed will automatically generate test cases that may trigger violations of the traffic rules, and cover different ways of violating the traffic rules. 
% The idea is to keep evolving a test suite due to the robustness of the test cases against the specifications, i.e., the traffic rules and the violation coverage measure as the objective functions. 

% \todo{Present details of the fuzzing algorithms here. They can be similar to the ones in the other paper.}


\begin{algorithm}[t]
\caption{Fuzzing for violations.}\label{alg:fuzzing_failure}
\small
\KwIn{A SCENEST \cite{} script $S$ with traffic rule $\Phi$; population size~$n$; crossover and mutation probabilities $c_p$ and $m_p$; top criteria , and the maximal number of generations $M$.}
\KwOut{A set of test cases that violate $\Phi$: $\mathbb{S}$.}
% \tcc{Step 0: Initialization}
 $\mathbb{S}=\emptyset$\;
Evaluate the initial test case described in $S$\;
\If{$S$ violates $\Phi$}{ $\mathbb{S} = \{S\}$;}
Generate initial test cases randomly based on $S$, denoted as $G_0=\{s_1,\ldots,s_n\}$, where $G_0[i] = s_i$\;
% Encoding the initial population $G_0$\;
\Repeat{\emph{Generation number reach M} or the top criteria has been satisfied}
{
    % \tcc{Test Case Evaluation}
    % \For{$i\in \{1,2,\ldots, n\}$}{
    % Simulate $s_i\in G_0$ using a simulator and obtain a trace $\pi_i$\;
    Execute $s_i$ in $G_0$ via simulation and obtain trace $\pi_i$\;
    Compute the robustness $\rho(\Phi, \pi_i)$\;
    \If{$\rho(\Phi, \pi_i)<0$}{
            $\mathbb{S} = \mathbb{S} \cup \{s_i\}$
        }
    % }
    % \tcc{Step 1: Selection}
    % $G_n=\{s_{i0}\}$, where $s_{i0}$ is the test case in $G$ with the lowest robustness\;
    $G = \emptyset$\;
    Sort $G_0$ according to $\rho(\Phi, \pi_i)$ in ascending order\;
    % \Repeat{$|G|<n$}
    \While{$|G|<n$}
    {
        Select two test cases by random, one from the first half of the sorted $G_0$ and another from $G_0$\;
        % Randomly select another test case, say $s_{i2}$, from $G_0$\;
        Add the test case with lower robustness to $G$;
        % $k = \argmin\limits_{i1, i2} \{\rho(\Phi, \pi_{i1}), \rho(\Phi, \pi_{i2})\}$\;
        % $G = G \cup \{s_k\}$\;
    }
    % \tcc{Step 2: Crossover}
    %  Sort $G$ according to $\rho(\Phi, \pi_i)$ in an ascending order\;
    $k = 1$\;
    \While{$k<n$}{
        Generate a random value $p \in [0,1]$\;
        \If{$p<c_p$}{
            $G[k], G[k+1] = Crossover(G[k], G[k+1])$\;
        }
        $k = k + 2$\;
    }
    % \tcc{Step 3: Mutation}
    \For{$k=\{1,2,\ldots, n\}$}{
        Generate a random value $p \in [0,1]$\;
        \If{$p<m_p$}{
            $G[k] = Mutation(G[k])$\;
        }
    }
    $G_0=G$\;}
    \Return $\mathbb{S}$.
\end{algorithm}

\begin{comment}
\begin{algorithm}[t]
\caption{Robustness Satisfaction}\label{alg:robust_satisfaction}
\small
\KwIn{AV simulator $A$; Assertion $\varphi$;A valid scenario $s$}
\KwOut{robustness value $v$}
Set up $A$ with the scenario $s$;\\
Running $A$ for xx mins and generate the trace $w$ by recording the signals every xx seconds;\\ 
Let $v:=\rho(\varphi,w,t)$;\\
\Return robustness value $v$
\end{algorithm}
\end{comment}

\subsection{Violation-Inducing Fuzzing}
\label{sec:failure-fuzzing}


% *****************

% We start with randomly generating a set of test cases according to $S$. That is, a test case is considered valid if and only if it satisfies $S$, i.e., the initial configuration must conform to $S$'s specified configuration and the trajectory must conform to constraints specified by $S$. \todo{We need to explain the details once the SCENEST language is completely defined.} Next, we simulate the test cases (using mature simulation environment such as APOLLO + LGSVL or Autoware + CARLA) to obtain a trace for each test case. Afterwards, we compute the robust of each trace against the negative of the assertion, which evaluates how far the trace is from violating the assertion. Note that a value 0 means that the assertion is violated. We sort the test cases according to the robustness value and return the first test case if its robustness is 0. Otherwise, we discard half of the test cases, i.e., those of larger robustness, and then generate new test cases through crossover and mutation. \todo{We need to explain how crossover and mutation are done.} This process continues until it times out. 

% *****************


The overall fuzzing algorithm for failures is shown in Algorithm ~\ref{alg:fuzzing_failure}.  
Note that the goal of the algorithm is to generate critical scenarios which may lead to violations of the traffic rules. The overall algorithm is a customized genetic algorithm (GA) which will output a set of critical scenarios that can be described by a script $S$ and violate traffic rules. The first step of the algorithm is to generate a test suite randomly based on the script $S$ as the initial generation. Then, we will produce the next generation via selection, crossover, and mutation. Every generation will give birth to the next generation until reach the predefined number of generations. 
Before introducing these steps, we start with describing the population encoding.
% In the sequel, we give a more detailed descriptions on each step. 
% \noindent \textbf{Evaluation on the initial test case.}
% Due to user's misunderstanding of the map or even mistakes, we cannot guarantee that the test case given in the script $S$ is always correct and feasible. For example, the initial and target positions of the ego vehicle are not located on lanes or are not connected in the given map.  In this case, we will select the path that is nearest to the initial (resp., target) position and connected to the target (resp., initial) position.
% Next, we will check whether the corrected test case satisfies the given assertion. Only when the corrected test case does not violate the given assertion $\Phi$, we perform the GA algorithm.

% \noindent \textbf{Population initialization.} 
% % We start with randomly generating a set of test cases according to $S$.
% Since the objective of failure fuzzing is to identity a test case that violates the given assertion, the generated population should be used to  verify the assertion. Hence, first of all, each test case in the population should have the same map and objects. For example, in the scenario described by the script in Section \ref{sec:scenest-example}, there are only three NPC vehicles, i.e., npc1, npc2, and npc3 on the map ``SanFrancisco''. So each test case in the initial population has and only has npc1, npc2 and npc3 on the map ``SanFrancisco''.  
% Second, we do not change the sequence of lanes that each object follows with. This is because users may just want to test the ADS when the objects move along the predefined paths. 
% Third, clipping functions are used to guarantee that the described motion of each object is feasible during initialization. For example, the motion of npc2 is described by a set of way-points, the clipping function will guarantee that the position of the latter way-point is farther than the previous ones.


\noindent \textbf{Population encoding.}
As illustrated in \cite{}, we describe a test case by depicting the ego vehicle, NPC vehicles, pedestrians, static obstacles, and the environment. To encode these objects, we will first figure the operable parameters of these objects. 
For the ego vehicle, the operable parameter is its starting point. Note that the destination will not mutate since it's the task to be tested and the effects of other parameters (e.g., vehicle type, vehicle color, and vehicle size) are trivial. 
For NPC vehicles and pedestrians, all the parameters except the speed at the destination are operable, since the speed at the destination is always zero.
For static obstacles and the environment, all the parameters in the language are operable.

These operable parameters are divided into six divisions: 
\emph{position, speed, type, color, daytime, and weather}. 
The division of position can be divided into three sub-divisions: vehicle position(i.e, ego position and NPC vehicles' positions), pedestrian position, and obstacle position. Note that the vehicle position is always within the lane or junction area, while pedestrians may move around the empty regions of the map, and obstacles can be placed at anywhere of the map (e.g, a basketball on the road, a meteorite on the roof, or a kite stuck in a tree). The division of speed can also be classified into vehicle speed and pedestrian speed due to different speed ranges. Similarly, the division of type can be divided into vehicle type, pedestrian type, and obstacle type since they have different list of values.

Among the above divisions, the value of position and speed are continuous, which leads to real-value encoding for vehicle position,  pedestrian position, obstacle position, vehicle speed, and pedestrian speed. 
The trajectory of NPC vehicles and pedestrians is defined by a sequence of states, including the initial and target state. Every state contains information of position and speed, we call every state among the trajectory a waypoint. 
Since the users may be interested in the specific trajectory of the NPC vehicles, we maintain the sequence of lanes although we can alter it.
Because vehicles are moving along lanes, we can translate the position of a vehicle in a waypoint into a lane position, allowing the encoding of each position to be described by its offset in the lane position format. Then, for every waypoint, the lane ID remains the same and the position and speed are encoded into a pair to form the chromosomes of vehicle position and vehicle speed.
Different from the vehicle position, the possible regions of pedestrian(or obstacle) position are larger as mentioned before, so we use coordinate positions to describe their locations. Each coordinate position is encoded as a gene.
The encoding of pedestrian speed is same as the vehicle speed. 
The position and speed pairs of all pedestrians are also concatenated sequentially to form the chromosome of the waypoint.

The divisions of type, color, and daytime are discrete values. We can treat each of them as a list of certain fixed values, so they are encoded as discrete vectors.

The division of weather is a dictionary variable, and its keys and values are the types of weather and the quantification of the weather type. Note that the value of weather is continuous and is within the range $[0,1]$.
% Note that if the value of a weather type variable is a predefined level label (e.g., small, middle), it will be transferred to a real value in range $[0,1]$.

% As an example, the encoding of the scenario described in Listing \ref{lst:scenario} is given in Appendix \ref{sec:algorithm}.



% On one hand, based on the scenario expression described in Section \ref{sec:scenest-expression}, each test case contains discrete and continuous variable. For example, object types (e.g., vehicle types, pedestrian types, and static obstacle types) and weather kinds are discrete variables, the position, speed, and heading are continuous variables. 
% % If some variable, such as color, can be either discrete or continuous variables, we will first transfer the discrete format to its corresponding continuous one and regard it as a continuous variable. 
% % Hence, each variable in a test case is either discrete or continuous. 
% For discrete variables, we apply the binary encoding, while for continuous variables, we apply real value encoding. 

% For example, for the scenario described in Section \ref{sec:scenest-example}, the speeds of the ego vehicle, npc1, npc2, and npc3 are encoded as a real-value vector $(v^0_0, v^1_0,v^1_1, v^2_0, v^2_1, v^2_2,v^2_3,v^2_4, v^3_0)$, where 
% $v_0^0$ is the initial speed of the ego vehicle corresponding to the initial state $\mathtt{ego\_init\_state}$; 
% $v^1_0$ and $v^1_1$ are the speed of npc1 corresponding to the initial state $\mathtt{npc1\_init\_state}$ and the way-point $\mathtt{npc1\_state}$; 
% $v^2_0$ is the initial speed of npc2 corresponding to the initial state $\mathtt{npc2\_init\_state}$, and $v^2_1 - v^2_4$ are the speeds corresponding to the four way-points described in $\mathtt{npc2\_states}$;
% and 
% $v^3_0$ is the initial speed of npc3 corresponding to the state $\mathtt{npc3\_init\_state}$.
% Note that for the speed of the ego vehicle, we can only customize its initial speed; for other movable objects, the speed at the destination state should be zero, so we do not need to encode the speed at the desination state.

% \noindent \textbf{Selection.}
% Based on the semantics of robustness, our GA algorithm prefers to select individuals with smaller robustness. In our algorithm, we use the 2-way tournament selection strategy to select test cases from the population.
% Each time we first randomly select two test cases from the original population $T_0$, and then the test case with smaller robustness is added to the new population $T$.
\noindent \textbf{Selection.}
The target of our algorithm is to generate test cases violating the traffic rules, i.e., with negative robustness, so we sort the population by their robustness in ascending order.
For every selection process, we first choose an individual from the first half of the population. Then, we select an individual from the overall population. For these two selected individuals, the individual with the lower score of robustness will be chosen.
We will repeat the selection process until a given number of parent populations are selected.
% Since our target is to generate test cases with negative robustness, we first sort the population according to their robustness in ascending order.
% The selection of an individual is described as follows. We first select an individual from the first half of the population and then select an individual from the whole population. Finally, the individual with lower robustness is selected from the two individuals. 
% Repeating the selection process, we can select a parent population with the given number of individuals.

\noindent \textbf{Crossover.}
% Crossover on positions may cause infeasible scenarios which violate the constraints.
In this work, to avoid the problem of infeasible scenarios, we abandon the crossover on the chromosomes of vehicle and pedestrian positions.


% For each pair of test cases, the crossover can be done only in the same category. 
% In theory, we can perform crossover for each category.
% However, crossover on positions may cause infeasible scenarios which violate the constraint described in Equation \ref{c6} in Definition \ref{trace}. 
% % For example, as shown in Fig. \ref{fig:infeasible_crossover}, position 1 and position 2 are the vehicle position encoding in two test cases, the displayed offsets in either position are located at the same lane. Clearly, after crossover, the path described in position 2' is infeasible since the third offset is less than the second one. 
% Hence, to guarantee the feasibility of the new individual, we do not perform crossover on the vehicle and pedestrian position chromosomes. 

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{images/infeasible_crossover.eps}
%     \caption{Crossover on position results in infeasible path.}
%     \label{fig:infeasible_crossover}
% \end{figure}



\noindent \textbf{Mutation.} 
The mutation is necessary for every division.
For division with continuous value, i.e., position, speed, and weather, we apply Gaussian mutation. We also apply the clipping function to avoid invalid values.
% To avoid invalid value, we apply clipping function to guarantee that all speeds are positive, no backward motion in the waypoints of NPC vehicles, and each weather quantification is in $[0, 1]$.
For divisions with discrete value, we apply random mutation, i.e., randomly select a value from a predefined set.

% We can do mutation for each category. 
% For continuous categories, i.e., position, speed, and weather, we apply Gaussian mutation. To guarantee the feasibility of motion, we need the clipping function to guarantee that all speeds are positive, no backward motion in the waypoints of NPC vehicles, and each weather quantification is in $[0, 1]$.  
% For discrete categories, we apply random mutation, i.e., randomly select one value from the corresponding set.

\subsection{Violation-Coverage Fuzzing}
There may be various ways of violating a traffic rule $\Phi$, so we define a specification-based violation coverage to evaluate the test sufficiency based on the number of atom elements $\varphi$ in $\Phi$ that could cause a violation of $\Phi$.
Note that the atom elements $\varphi$ here are can be either predicates of continuous variables (e.g. $Time \geq 20:00$, $ turnSignal \neq right$) nor Boolean values (e.g. $engineOn$, $stoplineAhead(realvalue)$).
We define the set of all the atom elements whose satisfaction will lead to the violation of $\Phi$ as $\Theta$. 
For a traffic rule $\Phi$, it's a combination of atom elements $\varphi$ in our language. 
In detail, traffic rules are the combinations of the following formulas: $\lnot x_1$, $x_1 \land x_2$, $x_1 \lor x_2$, $x_1 \to x_2$, $G\ x_1$, $F\ x_1$, $x_1\ U\ x_2$, and $X\ x_1$.
Therefore, we can define $\Theta$ as follows.
\begin{definition}\label{spec_coverage}
The set of atom elements $\Theta$ that cause violations to traffic rule $\Phi$ can be computed as follows. 
\begin{itemize}
    \item {\small$\Theta(x) = \{\lnot x\}$}; 
    {\small
    \item  $\Theta(x_1 \land x_2)$ $=$ $\Theta(x_1) \land N(x_2)\bigcup N(x_1)\land \Theta(x_2) \bigcup \Theta(x_1) \land \Theta(x_2)$;
    \item $\Theta(x_1 \lor x_2)$ $=$ $\Theta(x_1) \land \Theta(x_2)$;
    \item $\Theta(x_1 \to x_2)$ $=$ $N(x_1)\land \Theta( x_2)$;
    \item $\Theta(\lnot x_1)$ $=$ $N(x_1)$;
    \item $\Theta(G\ x_1) = F\ \Theta(x_1)$;
    \item $\Theta(F\ x_1) = G\ \Theta(x_1)$;
    \item $\Theta(x_1 U x_2) = (\Theta(x_1) \land \Theta(x_2)) \bigcup ((N(x_1) \land \Theta(x_2)) U (\Theta(x_1) \land \Theta(x_2)))$;
    \item $\Theta(X x_1) = X(\Theta(x_1))$}
\end{itemize}
where  $N(x) = x$, and the operations of two sets $A$ and $B$ can be described as follows:
{\small $A\land B= \{x_1\land x_2: \forall x_1\in A, \forall x_2\in B\}$, 
$F\ A = \{F\ x: \forall x \in A\}$, 
$G\ A = \{G\ x: \forall x \in A\}$, 
$X\ A = \{X\ x: \forall x \in A\}$, and 
$A\ U\ B = \{x_1\ U\ x_2: \forall x_1\in A, \forall x_2\in B\}$.}
\end{definition}

All the formulas that cause violations of traffic rule $x$ are in set $\Theta(x)$. Therefore, we define our violation coverage by the percentage of formulas in $\Theta(x)$ are satisfied, and the detailed definition is as follows. 
\begin{definition}
Given a set of scenarios $\mathbb{S}$ and a testing traffic rule~$x$, the violation coverage, denoted as $cov(\mathbb{S}, x)$, is defined as $cov(\mathbb{S}, x) = |\cup_{S\in \mathbb{S}} V(S)| / |\Theta(x)|$.
\end{definition}

Given the definition of specification-based violation coverage, we present our violation-coverage fuzzing algorithm in Algorithm \ref{alg:fuzzing_for_failuare_coverage}.
First of all, we generate the initial test cases randomly or use the violation test cases generated by Algorithm~\ref{alg:fuzzing_failure} as the initial test cases. Note that the violation test cases generated by Algorithm~\ref{alg:fuzzing_failure} are more recommended for initial test cases due to quicker convergence.
For every generation, we execute all the test cases in population and check whether the cases cover new violation atom elements.
We will add a test case to parents set $G'$ if and only if the test case covers new atom elements in set $\Theta(\Phi)$.
Note that the population of parents may not be enough for the predefined number, so we add random parents in this situation(Lines \ref{random_0}--\ref{random_1}).
With the parents set $G'$ selected, we apply crossover and mutation operation described in Section \ref{sec:failure-fuzzing} to obtain the next generation.
Repeating this process until all the atom elements in set $\Theta(\Phi)$ are covered.

% We first generate a set of initial test cases randomly.
% However, since failure test cases are rare, we may reuse the failed test cases generated by Algorithm~\ref{alg:fuzzing_failure} as the initial test cases.
% At each generation, we execute each test case and check whether its trace covers new failure predicates.
% Only when it covers new failure predicates will the test case be added to $T'$ to generate the next population (Lines \ref{add_0}--\ref{add_1}). 
% Note that there may not be enough test cases that can improve the failure coverage, so we randomly generate the rest test cases (Lines \ref{random_0}--\ref{random_1}).
% Finally, we apply the crossover and mutation operators described in Section \ref{sec:failure-fuzzing} to the new test cases $T'$ and generate the population of the next generation.



\begin{algorithm}[t]
\caption{Fuzzing for failure coverage.}\label{alg:fuzzing_for_failuare_coverage}
\small
\KwIn{A SCENEST \cite{} script $S$; a traffic rule $\Phi$; a population size $n$, and the maximal number of generations $M$}
\KwOut{A test suite}
Let $\Theta(\Phi)$ be the set of atom elements which will cause violation of $\Phi$\;
Let $\Theta_c(\Phi)=\emptyset$ be the set of covered atom elements of set $\Theta(\Phi)$\;
Let $G=\{s_1,\ldots,s_n\}$ be a set of random test cases or violation test cases generated by Algorithm~\ref{alg:fuzzing_failure}\;
\Repeat{\emph{Generation number reach M} or the coverage criteria has been satisfied}
{
    $G'=\emptyset$, $\Theta_c^i(\Phi)=\emptyset$\;
    \For{each $s_i$ in  $G$ }{
        Execute $s_i$ via simulation and obtain trace $\pi_i$\;
        Obtain the satisfied atom elements in $\Theta(\Phi)$: $\Theta_c(\Phi, s_i)$\;
        \If{$\Theta_c(\Phi, s_i)\setminus \Theta_c^i(\Phi) \neq \emptyset$\label{add_0}}{
            $G'=G'\cup \{s_i\}$; 
            $\Theta_c^i(\Phi) = \Theta_c^i(\Phi) \cup \Theta_c(\Phi, s_i)$;
        }\label{add_1}
    }
    $\Theta_c(\Phi)=\Theta_c(\Phi)\cup \Theta_c^i(\Phi)$\;
    \If{$|G'|\leq n$\label{random_0}}{
        Randomly generate $n-|G'|$ tests and add to $G'$\;
    }\label{random_1}
    Apply the crossover and mutation operators described in Section \ref{sec:failure-fuzzing} to $G'$ to generate the next population, denoted as $G$;
}
\end{algorithm}

% \subsection{Model-Coverage Fuzzing}
% Often we need to generate a test suite which demonstrates the AV has been thoroughly evaluated. The sufficiency of a test suite can be often measured using certain coverage criteria. In the following, we define multiple practical coverage criteria and then present a new fuzzing algorithm which generates a test suite that maximizes a given coverage. 

% % \paragraph{Model-based coverage} 

% As described in the \coolname, a script $S$ defines different \emph{types} of objects contained in a scenario, such as time and weather, NPC vehicles, pedestrians, and other static obstacles. 
% Each object is characterized by different \emph{features}. For example, the features to characterize weather can be rain, fog, and wetness.
% On one hand, we want to generate diverse test cases such that each possible feature value is tested for each object. 
% However, on the other hand, the combination of different features for each object will cause exponential increase in the number of test cases.
% In this paper, rather than focusing on each object, we consider features in terms of object types and generate test cases such that each possible feature value for an object type is tested in at least one object.  

% Given a simulator, a feature is either continuous or discrete. 
% For a continuous feature, we first divide the possible range into a set of disjoint intervals, and the coverage then is defined as the ratio of the number of visited intervals to the total number of intervals. 
% For a discrete feature, one simple way is to calculate the coverage as the ratio of the number of covered values to the number of supported values by the simulator. 
% However, if there are too many discrete values, we can also deal with discrete values like that for continuous values. 
% In the sequel, taking the LGSVL simulator as an example, we give the coverage of each feature in \coolname.

% Based on the syntax of \coolname, we have the following object types: time, weather, ego vehicle, NPC vehicle, pedestrian, and static obstacle. 
% \begin{itemize}[leftmargin=*]
%     \item \emph{Time}. There are two features: hour and minute. The sets  of values for hour and minute are $\{0, 1, \ldots, 23\}$ and $\{0, 1, 2, \ldots, 59\}$. Even though they are discrete features, two adjacent hours may not show significant difference. Moreover, for the same hour, difference values of minute also do not show great difference. Hence, for the time type, we only focus on the hour feature. We divide the values into 12 sets, each of which contain two adjacent hour values, starting from zero. Hence, the set of time feature values is $Cov_t=\{[2i,2i+1]: i\in \{0,1,\ldots, 5\}\}$. Given a scenario $s$, the time interval that its hour belongs to is denoted as $Cov_t(s) \in Cov_t$.
%     \item \emph{Weather}. Weather can be described by different features, such as fog, rain, and wetness. Suppose the features for weather is $W$. Each feature $w$ is quantified by a real value in $[0,1]$. In this work, for each weather feature $w$, the interval $[0,1]$ is divided into 7 intervals: $T_{w} =\{[0,0.2)_w$, $[0.2, 0.4)_w$, $[0.4, 0.6)_w$, $[0.6, 0.8)_w$, $[0.8, 1]_w$, $1_w\}$. Hence, the set of possible weather values is $Cov_W= \bigcup_{w\in W} T_w$. Given a scenario $s$, the weather conditions that it belongs to is denoted as $Cov_W(s) \subset{Cov_W}$.
%     \item \emph{Ego Vehicle}. For the ego vehicle, it can be mainly characterized by the vehicle type and the initial position. The set of possible vehicle types, denoted as $E_T$, is predefined before testing. It is determined either by the simulator or by users who can customize different vehicles in the simulator in advance. The initial position is a continuous variable. In this work, we evaluate the position in terms of its relative location on a lane. Given a lane, its lane length and start point are denoted as $s$ and $p_0$, respectively. Given an arbitrary point $p$ one the lane, its distance to $p_0$ is denoted as $d(p,p_0)$.
%     To evaluation of the point coverage of the lane, in this work, we divide the lane into three regions, i.e., $R_1=\{p: 0\leq d(p,p_0)<\frac{s}{3}\}$, $R_2=\{p: \frac{s}{3}\leq d(p,p_0)<\frac{2s}{3}\}$, and $R_3\{p: \frac{2s}{3}\leq d(p,p_0)<s$.
%     Hence, the set of position feature for the ego vehicle is $E_p = \{R_1, R_2, R_3\}$.
%     So the set of possible feature values for ego vehicle can be described as $Cov_E= E_T \cup E_p$.
%     Given a scenario $s$, the feature values of the ego vehicle is denoted as $Cov_E(s) = \{E_T(s), E_p(s)\} \subset{Cov_E}$.
%     \item \emph{NPC Vehicles}. Based on \coolname, an NPC vehicle can be described by its type and motion trajectory. Like the ego vehicle, the type of an NPC is predefined before testing, denoted as $NPC_T$. 
%     The motion trajectory can be described as a set of waypoints, including the initial and target positions of the vehicle. 
%     Note that each waypoint contains position and speed, except the target positions whose speeds are zero. 
%     Hence, given a script $S$, the set of all features' values for NPC vehicles can be defined as follow. First, we extract the lanes containing the defined waypoints in $S$, denoted as $\mathbb{L}$. Each lane $l$, $l\in \mathbb{L}$, is then divided into three disjoint segments, denoted as $L_l$. 
%     So the set of lane segments can be denoted as $NPC_L = \bigcup_{l\in \mathbb{L}} L_l$. 
%     The position coverage measures how many lane segments have been covered. 
%     Second, for each speed variable, we divide its range into three equal-length intervals, meaning the speed is slow, middle, and fast, respectively. We would like to each kind of speed is appeared in each lane segment in $NPC_L$. Hence, the coverage measures with respec to the motion of NPC vehicles can be described as $NPC_M = NPC_L \times \{slow, middle, fast\}$. Hence, the final set of possible feature values for NPC vehicles is $Cov_{NPC} = NPC_T \cup NPC_M$.
%     Given a vehicle $npc$, its feature values can be denoted as $Cov_{NPC}(npc) = NPC_T(npc) \cup NPC_M(npc)$.
%     Hence, the feature values in a scenario $s$ can be denoted as $Cov_{NPC}(s) = \bigcup_{npc \in s} Cov_{NPC}(npc)$.
%     \item \emph{Pedestrians}. Each pedestrian can also be described by the types and motions of pedestrians. However, the motion of a pedestrian can be any reasonable waypoint sequence. Hence, we focus on the pedestrian types. Similarly, suppose the predefined set of pedestrian types is $Ped_T$, then the set of all features' values can be described as $Cov_{ped} = Ped_T$.
%      The feature values of pedestrians in a scenario $s$ can be denoted as $Cov_{NPC}(s) = \bigcup_{ped \in s} \{Cov_{ped}(ped)\}\subset{Ped_T}$.
%     \item \empty{Static Obstacles}. Each static obstacle is defined by the type and position. Similar with the pedestrian, an obstacle can place anywhere in the map, so we do not consider the positions of static obstacles. Hence, the value set of features for pedestrians can be described as $Cov_{obs} = OBS_T$, where $OBS_T$ is predefined types by the simulator or customers. 
%      The feature values of pedestrians in a scenario $s$ can be denoted as $Cov_{obs}(s) = \bigcup_{obs \in s} \{Cov_{obs}(obs)\}\subset{OBS_T}$.
% \end{itemize}

% The set of all possible feature values is denoted as $Cov=Cov_t \cup Cov_W \cup Cov_E \cup Cov_{NPC} \cup Cov_{ped} \cup Cov_{obs}$.
% Given a scenario $s$, its covered values is calculated as 
% $Cov(s) = Cov_t(s) \cup Cov_W(s) \cup Cov_E(s) \cup Cov_{NPC}(s) \cup Cov_{ped}(s) \cup Cov_{obs}(s)$.
% Hence, the model coverage of a test suite $\mathcal{S}$ can be defined as follows. 
% \begin{definition}
% Given a test suite $\mathcal{S}$, its model coverage, denoted as $cov_m(\mathcal{S})$ can be defined as:
% \begin{equation*}
%     cov_m(\mathcal{S}) = \frac{|\bigcup_{s\in S} Cov(s)|}{|Cov|}
% \end{equation*}
% \end{definition}

% Based on the definition model coverage, the model-coverage fuzzing algorithm is described in Algorithm \ref{alg:fuzzing_for_model_coverage}. 
% \begin{algorithm}[t]
% \caption{Fuzzing for model coverage algorithm}\label{alg:fuzzing_for_model_coverage}
% \small
% \KwIn{A SCENEST script $S$; a population size $n$, and the maximal number of generations $G$}
% \KwOut{A test suite}
% Compute all possible feature values of $S$, denoted as $Cov$\;
% Let $T=\{s_1,\ldots,s_n\}$ be a set of random test cases generated from $S$\;
% Let $Cov_d=\emptyset$ be the set of all covered feature values during the testing\;
% \Repeat{\emph{timeout} or the coverage criteria has been satisfied}
% {
%     $T'=\emptyset$\;
%     \For{each $s_i$ in  $T$ }{
%         Compute the model coverage of $s_i$: $Cov_d^i$\;
%         \If{$Cov_d^i \setminus Cov_d \neq \emptyset$\label{add_0}}{
%             $T'=T'\cup \{s_i\}$;
%             $Cov_d = Cov_d \cup Cov_d^i$;
%         }\label{add_1}
%     }
%     \If{$|T'|\leq n$\label{random_0}}{
%         Randomly generate $n-|T'|$ test cases and add to $T'$\;
%     }\label{random_1}
%     Apply the crossover and mutation operators described in Section \ref{sec:failure-fuzzing} to $T'$ to generate the next population, denoted as $T$;
% }
% \end{algorithm}

% % \subsection{Model Coverage Experiments}
% % \paragraph{Analysis of Model-Coverage Fuzzing Algorithm.}
% % Table \ref{tab:model-coverage} shows the model coverage of our method and the random method. 
% % We find that there are not much difference on model coverage between the two methods. 
% % The reason is that in our method, each generation only maintain the test cases can improve the model coverage. However, after a few generations, there are no test cases that increase model coverage, so all test cases are generated randomly. Hence, the coverage of our method and the random method are similar. In the future, we will investigate more efficient methods to improve model coverage. 

% % \begin{table}[]
% % \caption{Model Coverage Measure of Different Methods}
% % \label{tab:model-coverage}
% % \begin{tabular}{|c|c|c|ccccc|}
% % \hline
% %  &     &      & \multicolumn{5}{c|}{Round}   \\ \cline{4-8} 
% % \multirow{-2}{*}{Scenario} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Total \\ Inputs\end{tabular}} & \multirow{-2}{*}{Method} 
% % & 1  & 2  & 3  & 4  & 5  \\ \hline
% % & & GA3  & 52 & 52 & 52 & 53 & 52 \\ \cline{3-8} 
% % \multirow{-2}{*}{S1}   & \multirow{-2}{*}{72}                                                      
% %   & Rand & 52 & 52 & 52 & 52 & 52 \\ \hline
% % & & GA3  & 46 & 46 & 46 & 45 & 45 \\ \cline{3-8} 
% % \multirow{-2}{*}{S2}       & \multirow{-2}{*}{69}                                                      
% %   & Rand & 45 & 45 & 45 & 45 & 45  \\ \hline
% % & & GA3  & 48 & 48 & 48 & 47 & 46  \\ \cline{3-8} 
% % \multirow{-2}{*}{S3}       & \multirow{-2}{*}{66}                                                      
% %   & Rand & 45 & 45 & 46 & 45 & 46  \\ \hline
% % & & GA3  & 47 & 47 & 47 & 47 & 47  \\ \cline{3-8} 
% % \multirow{-2}{*}{S4}       & \multirow{-2}{*}{66}                                                    
% %   & Rand & 44 & 44 & 44 & 44 & 44  \\ \hline
% % & & GA3  & 59 & 59 & 60 & 59 & 59  \\ \cline{3-8} 
% % \multirow{-2}{*}{S5}       & \multirow{-2}{*}{83}                                                     
% %   & Rand & 59 & 59 & 59 & 58 & 58  \\ \hline
% % & & GA3  & 44 & 44 & 44 & 44 & 44  \\ \cline{3-8} 
% % \multirow{-2}{*}{S6}       & \multirow{-2}{*}{59}                                                      
% %   & Rand & 44 & 44 & 44 & 44 & 44  \\ \hline
% % & & GA3  & 44 & 44 & 44 & 44 & 44  \\ \cline{3-8} 
% % \multirow{-2}{*}{S7}       & \multirow{-2}{*}{59}                                                     
% %   & Rand & 44 & 44 & 44  & 44 & 44  \\ \hline
% % & & GA3  & 45 & 46 & 46  & 45 & 45  \\ \cline{3-8} 
% % \multirow{-2}{*}{S8}       & \multirow{-2}{*}{62}                                                 
% %   & Rand & 45 & 45 & 45  & 45 & 45  \\ \hline
% % & & GA3  & 37 & 37 & 37  & 37 & 37  \\ \cline{3-8} 
% % \multirow{-2}{*}{S9}       & \multirow{-2}{*}{50}                                                      
% %   & Rand & 37 & 37 & 37  & 37 & 37  \\ \hline
% % \end{tabular}
% \end{table}

==> _old_Background.tex <==
\section{Background}
\label{sec:Background}
In this section we present some background knowledge
required for understanding the rest of this paper.

\subsection{Cornerstone of Simulation-Based Testing}
AVs are composed of three main parts: perception equipment~(e.g.~Camera, GPS, Radar), ADS, and chassis control~(e.g.~Wheel, Brake, Gas). The ADSs process sensory information obtained from perception equipment and pass control command to the chassis control of vehicles. We can treat ADSs as drivers of the AVs. For the simulation-based testing of AVs, the ADSs obtain the related sensor information from the simulator and then send back control information on time. The simulator will establish the corresponding environment based on the communication with ADSs. In this structure, the simulators treat the ADSs as black boxes. Existing platforms, such as LGSVL~\cite{rong2020lgsvl}+Apollo\cite{apollo60} and CARLA~\cite{dosovitskiy2017carla}+Autoware~\cite{autoware}, are all open source and available to the public.

\subsection{DSL of AVUnit}
\label{DSL}
DSLs are necessary for the descriptions of scenarios across different simulators. The existing DSLs~\cite{althoff2017commonroad, queiroz2019geoscenario, fremont2019scenic, openscenario1} provide different ways of specifying a scenario. 

In this work, we implement the DSL of AVUnit~\cite{AVUnit2021} for the description of scenarios. AVUnit specifies the motions of NPC vehicles and pedestrians, and other environment related information, such as time and weather. Even though AVUnit only describes the motion task of the ego vehicle, the trajectory of the ego vehicle is determined by the ADS under test.
Hence, AVUnit describes a complete scenario.
The following are the supported objects of AVUnit:
\begin{itemize}
    \item \noindent \textbf{Ego Vehicle.} The ego vehicle ($egoVehicle$) is the autonomous vehicle equipped with the ADS under test. 
    In AVUnit, it is specified using the keyword \texttt{AV}, followed by some optional parameters: the initial state of the ego vehicle, its target state, and the $type$ of the vehicle. 
    \item \noindent \textbf{NPCs.} AVUnit allows the user to (optionally) specify not only their initial and target states but also their $motion$.
    \item \noindent \textbf{Pedestrian.} AVUnit allows the user to (optionally) specify not only their initial and target states but also their $motion$.
    \item \noindent \textbf{Static Obstacles.} AVUnit allows the user to (optionally) specify its position and type.
    \item \noindent \textbf{Environment.} AVUnit allows the user to (optionally) specify environments, i.e., weather and day of time
\end{itemize}



% \subsection{System Model}
% We define the system model based on \emph{trace}, which is a sequence of scenes. Here a scene is a snapshot, at some time instant, of the physical world (including the status of all agents) and the ADS world (including the perception results of these agents and traffic conditions by the ADS). 
 
% \begin{definition}
%     A scene is a tuple $(map, time, weather, ego,\\ npc, ped, obs)$ such that:
% \begin{itemize}
%     \item $map$ is the map data structure which contains all static information related to the map (see Detailed in Section~\ref{map});
%     \item $time$ is the current time;
%     \item $weather$ is the current weather; 
%     \item $ego$ is the status of the ego vehicle, including the position, orientation, velocity, and acceleration, as well as the ego vesicle's perception of the world;
%     \item $nps$ captures the status of each NPC vehicle, including position, orientation, velocity, acceleration, and size; 
%     \item $ped$ captures the status of each pedestrian $ped$, i.e., its position, orientation, velocity, acceleration, and size;
%     \item $obs$ captures the status of each static obstacle, i.e., its position and size;
%     \item $traffic$ captures the status of different traffic lights, such as traffic lights, stop sign, and speed limit;
% \end{itemize}
% \end{definition}

Note that each component has many details, i.e., composed of data variables. The examples of the DSL can be found in Appendix.


\begin{comment}
\subsection{Basic Operation of Genetic Algorithm} 
\label{sec:background_of_genetic_alg}
\todo{I don't think GA needs introduction. We can remove this part.}
Our law-breaking fuzzing algorithm must be customized for every DSL language and is based on the Genetic Algorithm. As shown in \emph{Genetic Algorithm}~\cite{mirjalili2019genetic}, the population encoding, mutation and crossover are basic operations of the genetic algorithm.
We customize the population encoding, mutation and crossover for the design of law-breaking fuzzing algorithm.


\noindent \textbf{Population encoding.}
As illustrated in Section~\ref{DSL},  we describe a test case by depicting the ego vehicle, NPC vehicles, pedestrians, static obstacles, and the environment. Each object has different operable parameters. For the ego vehicle, the operable parameter is its starting point. For NPC vehicles and pedestrians, all the parameters except the speed at the destination are operable, since the speed at the destination is always zero. For static obstacles and the environment, all the parameters in the DSL are operable.
% For static obstacles and the environment, all the parameters in the language are operable.
% As illustrated in AVUnit~\cite{AVUnit2021}, we describe a test case by depicting the ego vehicle, NPC vehicles, pedestrians, static obstacles, and the environment. To encode these objects, we will first figure the operable parameters of these objects. 
% For the ego vehicle, the operable parameter is its starting point. Note that the destination will not mutate since it's the task to be tested and the effects of other parameters (e.g., vehicle type, vehicle color, and vehicle size) are trivial. 
% For NPC vehicles and pedestrians, all the parameters except the speed at the destination are operable, since the speed at the destination is always zero.
% For static obstacles and the environment, all the parameters in the language are operable.

These operable parameters are divided into six divisions: 
\emph{position, speed, type, color, daytime, and weather}. 
The division of position can be divided into three sub-divisions: vehicle position(i.e, ego position and NPC vehicles' positions), pedestrian position, and obstacle position. 
Note that the vehicle position is always within the lane or junction area, while pedestrians may move around the empty regions of the map, and obstacles can be placed at anywhere of the map (e.g, a basketball on the road, a meteorite on the roof, or a kite stuck in a tree). 
The division of speed can also be classified into vehicle speed and pedestrian speed due to different speed ranges. 
Similarly, the division of type can be divided into vehicle type, pedestrian type, and obstacle type.

Among the above divisions, the value of position and speed are continuous, which leads to real-value encoding for vehicle position,  pedestrian position, obstacle position, vehicle speed, and pedestrian speed. 
The trajectory of NPC vehicles and pedestrians is defined by a sequence of states, including the initial and target state. Every state contains information of position and speed, we call every state among the trajectory a waypoint and. 
% Since the users may be interested in the specific trajectory of the NPC vehicles, we maintain the sequence of lanes although we can alter it.
Because vehicles are moving along lanes, we can translate the position of a vehicle in a waypoint into a lane position, allowing the encoding of each position to be described by its offset in the lane position format. Then, for every waypoint, the lane ID remains the same and the position and speed are encoded into a pair to form the chromosomes of vehicle position and vehicle speed. The encoding for pedestrian(or obstacle) is the same except for the different regions of position.
% Different from the vehicle position, the possible regions of pedestrian(or obstacle) position are larger, so we use coordinate positions to describe their locations. 
% % Each coordinate position is encoded as a gene.
% The encoding of pedestrian speed is same as the vehicle speed. 
% The position and speed pairs of all pedestrians are also concatenated sequentially to form the chromosome of the waypoint. 
The divisions of type, color, and daytime are discrete values. 
% We can treat each of them as a list of certain fixed values, so 
They are encoded as discrete vectors.
The division of weather is a dictionary variable and the value of every key is encoded as a continuous value.
% , and its keys and values are the types of weather and the quantification of the weather type.
% Note that the value of weather is continuous and is within the range $[0,1]$.
% Note that if the value of a weather type variable is a predefined level label (e.g., small, middle), it will be transferred to a real value in range $[0,1]$.

\noindent \textbf{Crossover.}
% Crossover on positions may cause infeasible scenarios which violate the constraints.
For each pair of test cases, the crossover can be done only in the same category. 
In theory, we can perform crossover for each category.
In this work, to avoid the problem of infeasible scenarios, we abandon the crossover on the chromosomes of vehicle and pedestrian positions.


% For each pair of test cases, the crossover can be done only in the same category. 
% In theory, we can perform crossover for each category.
% However, crossover on positions may cause infeasible scenarios which violate the constraint described in Equation \ref{c6} in Definition \ref{trace}. 
% % For example, as shown in Fig. \ref{fig:infeasible_crossover}, position 1 and position 2 are the vehicle position encoding in two test cases, the displayed offsets in either position are located at the same lane. Clearly, after crossover, the path described in position 2' is infeasible since the third offset is less than the second one. 
% Hence, to guarantee the feasibility of the new individual, we do not perform crossover on the vehicle and pedestrian position chromosomes. 

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{images/infeasible_crossover.eps}
%     \caption{Crossover on position results in infeasible path.}
%     \label{fig:infeasible_crossover}
% \end{figure}
\noindent \textbf{Mutation.} 
The mutation is necessary for every division.
For division with continuous value, i.e., position, speed, and weather, we apply Gaussian mutation. We also apply the clipping function to avoid invalid values.
% To avoid invalid value, we apply clipping function to guarantee that all speeds are positive, no backward motion in the waypoints of NPC vehicles, and each weather quantification is in $[0, 1]$.
% For divisions with discrete value, we apply random mutation, i.e., randomly select a value from a predefined set.

% \noindent \textbf{Robustness Calculation for Coverage}
% The basic robustness calculation is defined in \ref{sec:semantics}.
% The mutation is necessary for every division.
% For division with continuous value, i.e., position, speed, and weather, we apply Gaussian mutation. We also apply the clipping function to avoid invalid values.
% To avoid invalid value, we apply clipping function to guarantee that all speeds are positive, no backward motion in the waypoints of NPC vehicles, and each weather quantification is in $[0, 1]$.
% For divisions with discrete value, we apply random mutation, i.e., randomly select a value from a predefined set.
\end{comment}
